Analytical Construction of CBF-Based Safety Filters for Simultaneous State and Input Constraints (Extended Version)

We revisit the problem explored in [1] of guaranteeing satisfaction of multiple simultaneous state constraints applied to a single-input, single-output plant consisting of a chain of n integrators subject to input limitations. For this problem setting, we derive an analytic, easy-to-implement safety filter which respects input limitations and ensures forward-invariance of all state constraints simultaneously. Additionally, we provide a straightforward extension to the multi-input, multi-output chained integrator setting, and provide an analytic safety filter guaranteeing satisfaction of arbitrarily many simultaneous hyperplane constraints on the output vector. Whereas the approach in [1] obtains maximal invariant sets, our approach trades off some degree of conservatism in exchange for a recursive safety filter which is analytic for any arbitrary n >= 1.

==> Sections/Intuition_Double_Integrator.tex <==
\section{Intuition: Double Integrator} \label{sec:intuition_double_integrator}

For intuition, consider the special case of Problem \ref{plm:simplified} with $n = 2$. We can intuitively think of this case as applying a force to a particle of unit mass to prevent it from crossing a barrier at $x_1 = \ubar{x}_1$. If the particle is not moving toward the barrier at time $t$, i.e. $x_2(t) \geq 0$, then $|x_2(t)|$ can be arbitrarily large without endangering the particle. However, suppose the particle is moving toward the barrier, i.e. $x_2(t) < 0$. Then, for any value of $x_1(t)$, it is possible for $|x_2(t)|$ to be large enough that the particle cannot avoid colliding even under maximum deceleration, i.e. $u(t) = \bar{u}$.

Quantitatively, we can define the particle's minimum stopping distance at time $t$, $x_{stop}(t)$, as the distance from the barrier such that, if $x_2(t) < 0$ and $u(\tau) = \bar{u} \ \forall \tau \geq t$, the particle will eventually arrive at the barrier with zero speed. It can be shown that the minimum stopping distance at time $t$ is given by
\begin{equation} \label{eqn:min_stopping_distance}
    x_{stop}(t) = \frac{x_2(t)^2}{2\bar{u}}.
\end{equation}
Then, we can prevent the particle from crossing the barrier at $x_1 = \ubar{x}_1$ by enforcing the state constraint
\begin{equation} \label{eqn:min_stopping_dist_criterion_1}
    \begin{cases} x_1(t) - \ubar{x}_1 \geq 0, & x_2(t) \geq 0 \\ x_1(t) - \ubar{x}_1 \geq x_{stop}(t), & x_2(t) < 0 \end{cases}\ \forall t \geq 0
\end{equation}
which, while the constraint is enforced, is equivalent to
\begin{equation} \label{eqn:min_stopping_dist_criterion_2}
    x_2(t) \geq -\sqrt{2\bar{u}(x_1(t) - \ubar{x}_1)}\ \forall t \geq 0.
\end{equation}

As $x_{stop}$ is a nonnegative quantity, it is clear that $x_1 - \ubar{x}_1 \geq x_{stop}$ implies $x_1 \geq \ubar{x}_1$. Furthermore, by the definition of $x_{stop}$, at every time $t$ we know that applying $u(\tau) = \bar{u}\ \forall \tau \geq t$ will ensure that the particle never crosses the barrier. Rearranging \eqref{eqn:min_stopping_dist_criterion_2}, it is thus clear that
\begin{equation} \label{eqn:double_integrator_ICCBF}
    h(\vec{x}) = x_2 + \sqrt{2\bar{u}(x_1(t) - \ubar{x}_1)}
\end{equation}
is an input-constrained CBF \cite{agrawal2021ICCBFs} for the state constraint in \eqref{eqn:state_constraints_simple} and thus that the filter
\begin{equation} \label{eqn:example_safety_filter}
    \dot{h}(t) = u(t) + \frac{\bar{u}x_2(t)}{\sqrt{2\bar{u}(x_1(t) - \ubar{x}_1)}} \geq -\alpha(h(t))\ \forall t \geq 0
\end{equation}
for some $\alpha \in \calK_\infty$ ensures forward-invariance of $S_1$.
